Stochastic additive manufacturing simulation: from experiment to surface roughness and porosity prediction

Deterministic computational modeling of laser powder bed fusion (LPBF) process fails to capture irregularities and roughness of the scan track, unless expensive powder-scale analysis is used. In this work we developed a stochastic computational modeling framework based on Markov Chain Monte Carlo (MCMC) capable of capturing the irregularities of LPBF scan. The model is calibrated against AFRL single track scan data using a specially designed tensor decomposition method, i.e., Higher-Order Proper Generalized Decomposition (HOPGD) that relies on non-intrusive data learning and construction of reduced order surrogate models. Once calibrated, the stochastic model can be used to predict the roughness and porosity at part scale at a significantly reduced computational cost compared to detailed powder-scale deterministic simulations. The stochastic simulation predictions are validated against AFRL multi-layer and multitrack experiments and reported as more accurate when compared with regular deterministic simulation results.

==> table1.tex <==
\begin{table}[t!]
\vspace{-1mm}
\centering
\scalebox{0.8}{
\begin{tabular}{c|cc|cc|cc}
\toprule
\multirow{2}{*}{Method}              & \multicolumn{2}{c|}{\textbf{UT-Zappos50K}} & \multicolumn{2}{c|}{\textbf{Wider Attribute}} & \multicolumn{2}{c}{\textbf{CUB-200-2011}} \\
                                     & Top-1 Acc.              & Top-5 Acc.              & Top-1 Acc.            & Top-5 Acc.            & Top-1 Acc.               & Top-5 Acc.               \\ \midrule \midrule \multicolumn{7}{c}{\it (Supervised) Labels + Cl-InfoNCE} \\ \midrule
SupCon~\citep{khosla2020supervised}      & 89.0$\pm$0.4                & 99.4$\pm$ 0.3              & 49.9$\pm$0.8             & 76.2$\pm$0.2             & 59.9$\pm$0.7                & 78.8$\pm$ 0.3               \\ \midrule \midrule \multicolumn{7}{c}{\it   (Weakly-supervised) Attributes-Determined Clusters + Cl-InfoNCE} \\ \midrule
Ours      & 84.6$\pm$0.4                & 99.1$\pm$0.2               & 45.5$\pm$0.2            & 75.4$\pm$0.2             & 20.6$\pm$ 0.5               & 47.0$\pm$0.5                \\
%\midrule \midrule \multicolumn{7}{c}{\it Self-supervised Representation Learning (clustering-based, $Z=$ unsupervised clusters)} \\ \midrule \midrule
%$^\ddagger$SwAV~\citep{caron2020unsupervised}   & xxx$\pm$xxx                & xxx$\pm$xxx               & xxx$\pm$xxx             & xxx$\pm$xxx             & xxx$\pm$xxx               & xxx$\pm$xxx   \\ [1mm]
%$^\dagger$PCL~\citep{li2020prototypical} & 82.4$\pm$0.5               & xxx$\pm$xxx               & 41.0$\pm$0.4             & xxx$\pm$xxx             & 14.4$\pm$0.5               & xxx$\pm$xxx                \\[1mm]
%$^\dagger$K-means Clusters + Cl-InfoNCE (ours)     & 84.5$\pm$0.4                & xxx$\pm$xxx               & 43.6$\pm$0.4         & xxx$\pm$xxx             & 17.6$\pm$0.2               & xxx$\pm$xxx \\
 %\midrule \midrule \multicolumn{7}{c}{\it Self-supervised Representation Learning (non-clustering-based, $Z=$ instance id)} \\
  \midrule \midrule \multicolumn{7}{c}{\it  (Self-supervised) Instance-ID + Cl-InfoNCE} \\
 \midrule
    SimCLR~\citep{chen2020simple} & 77.8$\pm$1.5                & 97.9$\pm$0.8               & 40.2$\pm$0.9             & 73.0$\pm$0.3             & 14.1$\pm$ 0.7               & 35.2$\pm$0.6            \\\bottomrule
\end{tabular}
}
\vspace{-1mm}
\caption{\small Experimental results for different supervision levels with the presented Cl-InfoNCE objective.
%under supervised (pre-training using label supervision), weakly supervised (pre-training using data attributes), and conventional self-supervised (pre-training using neither label supervision nor data attributes) setting.
%Except for the CMC approach, each setting refers to a particular cluster construction  ($Z = $  downstream labels, attributes-determined clusters, and instance ID).
%The methods presented in this table are either contrastive or predictive learning approaches.
For weakly-supervised methods that consider attributes-determined clusters, we report the best results by tuning the hyper-parameter $k$. The results suggest that, with the help of auxiliary information, we can better close the performance gap between supervised and self-supervised representations.
}
\label{tbl:attributes-supervision}
\vspace{-4mm}
\end{table}
